The Chronicles of RAG: The Retriever, the Chunk and the Generator

Retrieval Augmented Generation (RAG) has become one of the most popular paradigms for enabling LLMs to access external data, and also as a mechanism for grounding to mitigate against hallucinations. When implementing RAG you can face several challenges like effective integration of retrieval models, efficient representation learning, data diversity, computational efficiency optimization, evaluation, and quality of text generation. Given all these challenges, every day a new technique to improve RAG appears, making it unfeasible to experiment with all combinations for your problem. In this context, this paper presents good practices to implement, optimize, and evaluate RAG for the Brazilian Portuguese language, focusing on the establishment of a simple pipeline for inference and experiments. We explored a diverse set of methods to answer questions about the first Harry Potter book. To generate the answers we used the OpenAI's gpt-4, gpt-4-1106-preview, gpt-3.5-turbo-1106, and Google's Gemini Pro. Focusing on the quality of the retriever, our approach achieved an improvement of MRR@10 by 35.4% compared to the baseline. When optimizing the input size in the application, we observed that it is possible to further enhance it by 2.4%. Finally, we present the complete architecture of the RAG with our recommendations. As result, we moved from a baseline of 57.88% to a maximum relative score of 98.61%.

==> common.tex <==
%\usepackage[normalem]{ulem}
\usepackage{color}
%\usepackage[T1]{fontenc}

% Uso: \comando{texto}, onde 'comando' pode ser 'entra', 'sai', 'rever', 'todo' 
%      ou 
%      \comando[nota adicional]{texto} 

\newcommand{\entra}[2][]{%
   {\color{blue}#2}%
   \ifx&#1&%
      {}% #1 is empty
    \else%
      \footnote{{\color{blue}(entra):} #1}% #1 is nonempty
    \fi%
}%

\newcommand{\sai}[2][]{%
   {\color{black}\sout{#2}}%
   \ifx&#1&%
      {}% #1 is empty
    \else%
      \footnote{{\color{black}(sai):} #1}% #1 is nonempty
    \fi%
}%

\newcommand{\rever}[2][]{%
   {\color{magenta}#2}%
   \ifx&#1&%
      {}% #1 is empty
    \else%
      \footnote{{\color{magenta}(rever):} #1}% #1 is nonempty
    \fi%
}%

\newcommand{\todo}[2][]{%
   {\color{red}[\textbf{TODO}: \textit{#2}]}%
   \ifx&#1&%
      {}% #1 is empty
    \else%
      \footnote{{\color{red}[(todo):} #1]}% #1 is nonempty
    \fi%
}%

\newcommand{\etal}{{\it et al.}}



==> texts/retrievers_bkp.tex <==
\section{Advanced Experiments}
%\ Até esta estapa, os estudos e experimentos apresentados na seção \ref{sec:experiments} tiveram desempenho insatisfatório, com uma degradação de pelo menos $20\%$ em relação ao máximo relativo.

The studies and experiments outlined in section \ref{sec:experiments} have shown unsatisfactory performance, marked by a degradation of at least $20\%$ compared to the peak relative performance. Therefore, in this section, we explore various search approaches for the RAG, recognizing that the quality of the retriever is a crucial factor in enhancing performance for this type of problem. While reviewing retrieval methods, we conducted an evaluation covering both sparse and dense search. In pursuit of code debugging flexibility and easier customization at each stage, we chose not to utilize a RAG framework (like LangChain our Llama-Index). For a comprehensive guide on debugging RAG, refer to \cite{build_RAG_ANYSCALE}.

 %\Nesta seção, investigamos diferentes abordagens de busca para o RAG, pois sabemos que a qualidade do retriever é  ponto-chave para a melhoria de desempenho nesse tipo de problema. Durante a análise dos buscadores, realizamos uma avaliação que incluiu tanto buscadores esparsos quanto densos.

 %\Buscando maior flexibilidade na depuração do código e maior personalização de cada etapa, optamos por não utilizar o framework do Llama-Index. Um trabalho detalhado sobre debug de RAG pode ser encontrado em \cite{build_RAG_ANYSCALE}.

%\ nós seguindos os mesmo passos de debug do trabalho citado?

\subsection{Retrievers}
\label{sec:retrievers}

%\No grupo dos buscadores esparsos, destacamos o BM25, uma técnica que se baseia em ponderações estatísticas para avaliar a relevância entre termos de busca e documentos. O BM25 utiliza uma função de pontuação que considera a frequência dos termos e a extensão dos documentos, proporcionando uma abordagem eficiente para recuperar informações relevantes.

In the category of sparse retrievers, we emphasize the BM25, a technique grounded in statistical weighting to assess relevance between search terms and documents. BM25 employs a scoring function that takes into account term frequency and document length, offering an efficient approach for retrieving pertinent information. In the BM25 ranking function, \(k_1\) and \(b\) are parameters shaping term saturation and document length normalization, respectively. The BM25 formula integrates these parameters to score the relevance of a document to a query, offering flexibility in adjusting \(k_1\) and \(b\) for improving performance in different retrieval scenarios.

%\Por outro lado, ao explorar os buscadores densos, temos duas abordagens distintas: bi-encoder e cross-encoder. O bi-encoder realiza a codificação independente de consultas e documentos, gerando representações vetoriais separadas antes de calcular a similaridade. Por outro lado, o cross-encoder adota uma abordagem mais integrada, já que a codificação leva em consideração simultaneamente a consulta e o documento, permitindo uma avaliação mais contextualizada da relevância.

On the other hand, when exploring dense retrievers, we often encounter  approaches like bi-encoder and cross-encoder. The bi-encoder independently encodes queries and documents, creating separate vector representations before calculating similarity. In contrast, the cross-encoder takes a more integrated approach by considering both the query and the document simultaneously during encoding, enabling a more context-aware evaluation of relevance.

%\Como comentado, bi-encoder e cross-encoder oferecem perspectivas distintas na busca por informações, sendo assim, dependendo do cenário de aplicação, cada uma possui suas próprias vantagens e desvantagens. Por exemplo, o bi-encoder pode ser inicializado de maneira offline, onde os embeddings dos documentos são calculados previamente, e apenas o embedding da consulta é calculado em tempo de busca, reduzindo a latência. Já na abordagem cross-encoder, como consulta e documento são vistos pelo modelo ao mesmo tempo durante o tempo de busca, temos uma latência maior. No entanto, espera-se alcançar um melhor desempenho com essa técnica \cite{monobert}, \cite{monot5}. Os cross-encoder são frequentemente utilizados como um segundo estágio da busca, onde um estágio inicial com menos latência reduz a quantidade de documentos que serão enviados para ele. Este, por sua vez, irá reordenar os documentos recebidos.

As mentioned earlier, bi-encoder and cross-encoder offer distinct perspectives in information retrieval. Depending on the application scenario, each has its own set of advantages and disadvantages. For instance, the bi-encoder can be initialized offline, with document embeddings calculated beforehand and only the query embedding calculated at search time, reducing latency. On the other hand, in the cross-encoder approach, since the model views both the query and document simultaneously during search, we experience higher latency. However, an improvement in performance is expected when using this technique \cite{monobert}, \cite{bert_and_beyond}. Cross-encoders are often employed as a second stage in search, where an initial stage with lower latency reduces the number of documents sent to it and, subsequently, it reorders the received documents.

%/ Tais modelos são capazes de codificar relações semânticas entre pares de consultas e documentos. Isso acontece pois a consulta e o documento são enviados em conjunto para o modelo, que irá gerar um score conforme a relevância pairwise de entrada. Para uma determinada busca, os documentos são então ordenados por esse score de forma decrescente. 

Figure \ref{fig:bi_and_cross_encoders} Cross-Encoder tend to be superior compared with Bi-Encoder for Information Retrieval tasks \cite{cross_rank_ref_1, cross_rank_ref_2}.

\begin{figure}[htb!]
\centering
\includegraphics[width=0.99\linewidth]{pics/bi_and_cross_encoders.png} 
\caption{Bi-Encoder and Cross-Encoder Architecture}
\label{fig:bi_and_cross_encoders}
\end{figure}

%/ tem alguma referencia? # https://www.sbert.net/examples/applications/cross-encoder/README.html

%/ Em nossos experimentos com buscadores, nossa avaliação busca mensurar, a partir de uma pergunta $_i$, se o chunk$_i$ figura entre as posições top-k por meio do recall. No entanto, observamos que essa métrica se limita a verificar a presença ou ausência do chunk$_i$ nas primeiras posições, sem considerar se ele está na primeira ou última posição dentro do intervalo avaliado. Para contornar essa limitação, optamos por incorporar o Mean Reciprocal Rank nas top 10 posições em nossa análise (MRR@10), essa métrica atribui maior valor quando os chunks mais relevantes são recuperados nas primeiras posições \cite{mrr}.

%\ talvez seria interessante colocar as formulas de calculo de cada um

In our experiments with retrievers, our evaluation aims to measure, based on a query $_i$, whether chunk$_i$ ranks among the top-k positions through recall. However, we note that this metric is confined to assessing the presence or absence of chunk$_i$ in the early positions, without considering whether it is in the first or last position within the evaluated range. To address this limitation, we chose to incorporate Mean Reciprocal Rank in our analysis (MRR). This metric assigns higher value when the most relevant chunks are retrieved in the early positions \cite{mrr} and was measured on top-10 retrieved chunks.

%\Os resultados alcançados com os diferentes buscadores são apresentados na Tabela \ref{tab:topk_retrieved}.

The results achieved with the various retrievers are presented in Table \ref{tab:topk_retrieved}.
 
\begin{table}[htbp]
\caption{Retriever comparison.}
\centering\centering\resizebox{0.7\textwidth}{!}{
\begin{tabular}{cccccc}
\hline
\textbf{Metrics}  & \textbf{ADA-002} &\textbf{Custom ADA-002} & \textbf{Hybrid} & \textbf{BM25}  & \textbf{Reranker}\\ \hline
MRR@10               & 0.565            & 0.665                 & 0.849           &    0.879        & 0.919          \\
R@3                  & 0.628            & 0.735                 & 0.921           &    0.914        & 0.971          \\
R@5                  & 0.692            & 0.835                 & 0.943           &    0.971        & 0.985          \\
R@7                  & 0.750            & 0.871                 & 0.964           &    0.985        & 0.992          \\
R@9                  & 0.814            & 0.921                 & 0.978           &    0.985            & 1              \\
\hline
\end{tabular}
}
\label{tab:topk_retrieved}
\end{table}

%\ A seguir temos mais detalhes de cada buscador utilizado.

Next, we provide more details about each retriever used.

\subsection{BM25}

%\Devido à facilidade de uso do BM25, acreditamos que sua inclusão para o teste de retrievers é sempre bem-vinda na avaliação de RAGs.
%\ acho que só facilidade é um argumento fraco. Seria errado falar que ele é um excelente "baseline", que muitos trabalhos usam como baseline comparativo e citar alguns? 

%\Um trabalho que segue a mesma linha de raciocínio, mas para uma diferente aplicação, é encontrado em \cite{bm25_baseline}, que demonstra os benefícios do uso desse algoritmo para estabelecer um baseline robusto. Como o nosso dado tem características semelhantes ao dataset \texttt{SQuAD} é esperado que muitas palavras da pergunta estivessem presentes no chunk, o que contribui para o desempenho favorável do BM25.

%\O desempenho também é influenciado pela escolha do pacote BM25 a ser utilizado. Neste trabalho, utilizamos a implementação do pacote Pyserini \cite{pyserini} em todos os experimentos, com valores de K1=0.82 e b=0.68. A implementação de BM25 do Pyserini possui etapas de pré-processamento como stemming e remoção de stop words específicos por idioma. Para efeitos de comparação, incluímos os resultados obtidos utilizando o \texttt{rank-bm25} (Okapi BM25) \cite{rankBM25}, implementação básica (sem pré-processamento) e popular em Python e integrado a bibliotecas como LangChain e llama-index; resultados podem ser vistos na tabela \ref{tab:bm25_compare}.

%\ I think ease of use alone is a weak argument. Would it be wrong to say that it is an excellent "baseline," widely employed in comparative studies, and cite some examples?

Due to the user-friendly nature of BM25, we believe its inclusion for retriever testing is always a welcome addition in RAG evaluations. A study that aligns with the same reasoning, albeit for a different application, can be found in \cite{bm25_baseline}, which illustrates the benefits of employing this algorithm to establish a robust baseline. Given that our data shares similarities with the \texttt{SQuAD} dataset, it is expected that many words from the query would be present in the chunk, contributing to the favorable performance of BM25.

Performance is also influenced by the choice of the BM25 package. In this work, we utilized the Pyserini package implementation \cite{pyserini} in all experiments, with \(k_1\)=0.82 and \(b\)=0.68. Pyserini's BM25 implementation incorporates preprocessing steps such as stemming and language-specific stop word removal. For the sake of comparison, we included results obtained using \texttt{rank-bm25} (Okapi BM25) \cite{rankBM25}, a basic implementation without preprocessing that is widely used in Python and integrated into libraries like LangChain and llama-index. The results can be seen in Table \ref{tab:bm25_compare}.

\begin{table}[htbp]
\caption{Comparison between BM25 packages.}
\centering\centering\resizebox{0.6\textwidth}{!}{
\begin{tabular}{cccc}
\hline
\textbf{Recall@k}  & \textbf{Okapi BM25} & \textbf{Pyserini BM25} & \textbf{Pyserini Gain (\%)} \\ \hline
3                  &  0.742              &  0.914                 & 23.1                \\
5                  &  0.828              &  0.971                 & 17.2                \\
7                  &  0.850              &  0.985                 & 15.8                \\
9                  &  0.892              &  0.985                 & 10.4                \\
\hline
\end{tabular}
}
\label{tab:bm25_compare}
\end{table}

\subsection{ADA-002}
%\ A OpenAI não divulga muitos detalhes da arquitetura do ADA-002, porém, utilizamos esse modelo na busca como se fosse uma configuração bi-encoder: são construídas representações vertoriais para todos os documentos disponíveis e, para cada pergunta de entrada, seu embedding é calculado em tempo de busca e então a similaridade entre pergunta e documentos é aferida com similaridade de coseno. Devido à falta de maiores detalhes do modelo, podemos nos referir a essa abordagem apenas como busca vetorial.

OpenAI does not disclose extensive details about the ADA-002 architecture; however, we employed this model in retrieval as a bi-encoder: vector representations are constructed for all available documents, and for each input query, its embedding is computed at search time. Subsequently, the similarity between the question and documents is assessed using cosine similarity.

\subsection{Custom ADA-002}
%/A customização de embeddings não se restringe apenas aos embeddings da OpenAI; é uma técnica aplicável a outros embeddings do mesmo tipo. Há uma variedade significativa de abordagens para otimizar uma matriz, sendo uma delas a aplicação da Multiple Negative Ranking Loss, conforme apresentado no artigo "Efficient Natural Language Response Suggestion for Smart Reply", Seção 4.4 \cite{mnrloss}. No entanto, dado nosso atual foco em simplicidade, reservaremos a exploração dessa técnica para trabalhos futuros. Neste momento, optaremos por utilizar a Mean Squared Error (MSE) Loss.

%/Para a etapa de fine-tuning, é necessário contar com dois tipos de amostras:

%\\begin{itemize}
%\    \item positives: [pergunta$_i$, chunk$_i$, $label =1$]
%\    \item negatives: [pergunta$_i$, chunk$_j$, $label=-1$], para $i\neq j$
%\\end{itemize}

%/Frequentemente, como é o caso do nosso dataset, apenas os exemplos positivos estão disponíveis. No entanto, por meio de um embaralhamento simples e aleatório, é possível gerar exemplos negativos. Demonstrando confiança no transfer-learning, verificamos que poucos exemplos foram suficientes.  Nosso dataset final consistiu em aproximadamente $400$ exemplos, mantendo uma proporção de $1:3$ entre exemplos positivos e negativos.

%/Os hiperparâmetros que exercem maior impacto no desempenho incluem a learning rate, batch size e o número de dimensões na matriz de projeção. O modelo ADA-002 possui $1536$ dimensões, e a matriz de projeção é de tamanho $1536\times\mathrm{N}$, onde $\mathrm{N}\in \{1024,2048,4096\}$. Em nossos experimentos, observamos que $2048$ dimensões resultaram na melhor acurácia.

Embedding customization is not limited solely to OpenAI's embeddings; it is a technique applicable to other embeddings of the same kind. There is a significant variety of approaches to optimize a matrix, with one of them being the application of Multiple Negative Ranking Loss, as presented in the article "Efficient Natural Language Response Suggestion for Smart Reply," Section 4.4 \cite{mnrloss}. However, given our current focus on simplicity, we will reserve the exploration of this technique for future work. At this moment, we choose to utilize the Mean Squared Error (MSE) Loss.

For the fine-tuning stage, it is necessary to have two types of samples:

\begin{itemize}
\item positives: [question$_i$, chunk$_i$, $label =1$]
\item negatives: [question$_i$, chunk$_j$, $label=-1$], for $i\neq j$
\end{itemize}

Often, as is the case with our dataset, only positive examples are available. However, through a simple and random shuffling, it is possible to generate negative examples. Demonstrating confidence in transfer learning, we found that a few examples were sufficient. Our final dataset consisted of approximately $400$ examples, maintaining a $1:3$ ratio between positive and negative examples.

The hyperparameters that exert the most significant impact on performance include the learning rate, batch size, and the number of dimensions in the projection matrix. The ADA-002 model has $1536$ dimensions, and the projection matrix is of size $1536\times\mathrm{N}$, where $\mathrm{N}\in {1024,2048,4096}$. In our experiments, we observed that $2048$ dimensions resulted in the best accuracy.

%\ Seria interessante colocar uma tabela ou grafico com esses resultados?

%/Este tipo de fine-tune demanda baixo recurso de GPU, com um tempo de treinamento de aproximadamente $5$ minutos usando a GPU A100. O modelo em si é simples, consistindo em uma matriz com dropout (para mitigar overfitting), seguida pela função de ativação tangente hiperbólica, que proporcionou ganhos adicionais de acurácia no conjunto de treinamento.

%/Ao analisar a similaridade cosseno entre as classes positivas e negativas, podemos observar a "sombra" compartilhada pelos histogramas. Em um cenário ideal, desejamos que as classes sejam disjuntas para garantir uma definição nítida do espaço. A Figura \ref{fig:ada_cos_sim} ilustra uma sombra significativa no embedding antes do treinamento, enquanto a Figura \ref{fig:custom_ada_cos_sim} mostra o resultado após o treinamento. Ambos os gráficos são derivados do conjunto de teste.

This type of fine-tuning requires low GPU resources, with a training time of approximately $5$ minutes using the A100 GPU. The model itself is straightforward, consisting of a matrix with dropout (to mitigate overfitting), followed by the hyperbolic tangent activation function, which provided additional accuracy gains in the training set.

When analyzing the cosine similarity between positive and negative classes, we can observe the "shadow" shared by the histograms. In an ideal scenario, we desire the classes to be disjoint to ensure a clear definition of space. Figure \ref{fig:ada_cos_sim} illustrates a significant shadow in the embedding before training, while Figure \ref{fig:custom_ada_cos_sim} shows the result after training. Both graphs are derived from the test set.

% \begin{figure}[htb!]
% \centering
% \includegraphics[width=0.99\linewidth]{pics/ADA002_cosine_sim.png} 
% \caption{Similaridade cosseno das classes positivos e negativos do embedding ADA-002, observe que existe muita interseção entre as classes, test accuracy (before training): $69.5\%$}
% \label{fig:ada_cos_sim}
% \end{figure}

\begin{figure}[htb!]
\centering
\includegraphics[width=0.99\linewidth]{pics/ADA002_cosine_sim.png} 
\caption{Cosine similarity of positive and negative classes in the ADA-002 embedding; note the significant overlap between the classes. Test accuracy \textit{(before training)}: $69.5\%$}
\label{fig:ada_cos_sim}
\end{figure}

% \begin{figure}[htb!]
% \centering
% \includegraphics[width=0.99\linewidth]{pics/ADA002_custom_cosine_sim.png} 
% \caption{Similaridade cosseno das classes positivos e negativos do embedding customizado, a interseção entre as classes é minima, , test accuracy (after training): $84.3\%$}
% \label{fig:custom_ada_cos_sim}
% \end{figure}

\begin{figure}[htb!]
\centering
\includegraphics[width=0.99\linewidth]{pics/ADA002_custom_cosine_sim.png} 
\caption{Cosine similarity of positive and negative classes in the customized embedding; the intersection between the classes is minimal. Test accuracy \textit{(after training)}: $84.3\%$}
\label{fig:custom_ada_cos_sim}
\end{figure}

\subsection{Hybrid Search}
% A técnica de busca híbrida se baseia em tentar aproveitar o melhor entre a busca esparsa e a busca densa. Dado uma pergunta, ambas as buscas são realizada paralelamente, gerando duas listas de documentos candidatos a respondê-la. Em seguida, o desafio consiste em combinar da melhor forma possível os dois resultados de forma que a lista final híbrida seja melhor do que as buscas individuais. Basicamente, podemos entender como um sistema de votação, onde cada buscador vota na relevância de um documento dada uma pergunta e ao final as opiniões são combinadas para gerar um resultado melhor. 

% Um algoritmo bastante utilizado para resolver esse tipo de problema é chamado de Reciprocal Rank Fusion (RRF). A partir de um conjunto $D$ de documentos e os resultados da busca realizada por diferentes métodos $r$ em $R$, para cada $d$ em $D$, podemos calcular o $RRF\_score (d \in D$) da seguinte maneira \cite{hybrid_fusion}:

The hybrid search technique aims to leverage the best of both sparse and dense search approaches. Given a question, both searches are conducted in parallel, generating two lists of candidate documents to answer it. The challenge then lies in combining the two results in the best possible way, ensuring that the final hybrid list surpasses the individual searches. Essentially, we can conceptualize it as a voting system, where each searcher casts a vote on the relevance of a document to a given question, and in the end, the opinions are combined to produce a better result.

A widely used algorithm to address this type of problem is known as Reciprocal Rank Fusion (RRF). For a document set $D$ and search results from different methods $r$ in $R$, for each $d$ in $D$, we can calculate the $RRF_{score} (d \in D)$ as follows \cite{hybrid_fusion}:

% \text{RRF_score}(d \in D) = \sum_{r \in R} \frac{1}{k + r(d)},
\begin{equation}
RRF_{score}(d \in D) = \sum_{r \in R} \frac{1}{k + r(d)},
\end{equation}

% Sendo que $1/r(d)$ é conhecido por reciprocal rank e $r(d)$ é a posição em que o documento $d$ foi retornado pelo mecanismo de busca $r$. O termo $k$ é adicionado para ajudar a controlar sistemas outliers.

Considering that $1/r(d)$ is known as the reciprocal rank, where $r(d)$ represents the position at which the document $d$ was retrieved by the search mechanism $r$. The term $k$ is introduced to assist in controlling outlier systems.

\begin{figure}[htb!]
\centering
\includegraphics[width=0.99\linewidth]{pics/hybrid_rank.png} 
\caption{Hybrid Search schema with k=1.}
\label{fig:hybrid}
\end{figure}

% A Figura \ref{fig:hybrid} representa essa abordagem tomando $k=1$. No exemplo, temos 4 chunks que foram retornados em diferentes ordens por dois métodos de busca, o BM25 (busca esparsa) e o Custom ADA-002 (busca densa). Para cada chunk é calculado o reciprocal rank score. Esses valores são então somados, formando um novo score. A lista final híbrida é uma ordenação dos chunks que utiliza esse novo score de forma decrescente.

% Em nossas abordagens, apenas o BM25 do Pyserini foi testado como buscador esparso, enquanto que ADA-002 e Custom ADA-002 foram testados como buscadores densos. A combinação híbrida que apresentou melhor resultado foi a que utilizou BM25 e Custom ADA-002.

Figure \ref{fig:hybrid} illustrates this approach with $k=1$. In the example, we have four chunks that were retrieved in different orders by two search methods, BM25 (sparse search), and Custom ADA-002 (dense search). The reciprocal rank score is calculated for each chunk. These values are then summed, creating a new score. The final hybrid list is an ordering of chunks that uses this new score.

In our experiments, only Pyserini's BM25 was tested as the sparse retriever, while ADA-002 and Custom ADA-002 were tested as dense retrievers. The hybrid combination that yielded the best results was the one that used BM25 and Custom ADA-002.

\begin{table}[htbp]
\caption{Retriever comparison. Where MRR is the Mean Recriprocal Rank metric and R@k is the Recall.}
\centering\centering\resizebox{0.7\textwidth}{!}{
\begin{tabular}{cccccc}
\hline
\textbf{Metric}  &  \textbf{Hybrid-BM25-ADA-002} & \textbf{Hybrid-BM25-Custom ADA-002}     \\ \hline
MRR@10             & 0.7578                         & 0.8496                              \\
R@3                & 0.8286                         & 0.9214                              \\
R@5                & 0.8786                         & 0.9429                              \\
R@7                & 0.9214                         & 0.9643                              \\
R@9                & 0.9571                         & 0.9786                              \\
\hline\end{tabular}}
\label{tab:topk_retrieved_ada}
\end{table}

\subsection{Reranker}
% Como visto anteriormente, a técnica de re-ranking se baseia em utilizar uma arquitetura com mais de um estágio durante o processo de busca. Na primeira etapa, normalmente é utilizado um buscador com bom recall para fazer um filtro inicial nos documentos a serem retornados. A partir dessa lista reduzida, tais documentos candidatos são então enviados para uma segunda etapa, de maior complexidade computacional, que irá reranqueá-los para alcançar um melhor desempenho final do sistema.

As seen earlier, the re-ranking technique relies on employing an architecture with more than one stage during the search process. In the first stage, a retriever with good recall is typically used to perform an initial filtering of the documents to be returned. From this narrowed-down list, these candidate documents are then sent to a second stage, which involves higher computational complexity, to re-rank them and achieve an improved final system performance. Re-rankers based on encoder-only models like BERT, also called cross-encoders, can be used on this task but encoder-decoder models can also be used and are called sequence to sequence rerankers.

\begin{figure}[htb!]
\centering
\includegraphics[width=0.99\linewidth]{pics/reranker.png} 
\caption{Reranker Pipeline, k within [3, 5, 7, 9]}
\label{fig:reranker}
\end{figure}

% Como primeiro estágio de busca foi utilizado o BM25, que recupera 50 documentos para serem reranqueados no segundo estágio conforme Figura \ref{fig:reranker} a seguir. No segundo estágio, ou estágio de reranking, utilizamos o modelo modelo \texttt{'unicamp-dl/mt5-base-en-pt-msmarco-v2'}, um reranker MonoT5 \cite{monot5} treinado em pares de queries e documents em inglês e português do dataset \cite{mmarco}.

% MonoT5 é um reranker que utiliza modelos T5 \cite{t5-google} para gerar scores de relevância entre um par de query e documento. Modelos T5 tratam todas tarefas como \textit{text-to-text}, o que exige algumas adaptações para a tarefa de similaridade entre query/documento. Durante o treino, utiliza-se o formato \texttt{Query: {query} Document: {document} Relevant:}, com labels \texttt{yes}, caso o documento seja relevante para a query, e \texttt{no}, caso contrário. Em tempo de inferência, utiliza-se o mesmo formato dos dados de treino para formatar pares de queries e documentos e alimentar o modelo, e é greedy decode um único token. O score é então obtido calculando-se o valor do softmax considerando apenas os tokens \texttt{no} e \texttt{yes}, e então selecionando o valor correspondente ao token \texttt{yes}. Note que os tokens \texttt{no} e \texttt{yes} são os tokens usados na versão disponibilizada por \cite{mmarco}, mas a publicação que introduziu a arquitetura MonoT5, \cite{monot5} utiliza os tokens \texttt{false} e \texttt{true}. A Figura \ref{fig:monot5} contém uma ilustração do processo de inferência da arquitetura MonoT5.

BM25 was employed as first-stage retrieval, retrieving 50 documents to be reranked in the second stage, as shown in Figure \ref{fig:reranker}. In the second stage, we utilized the model \texttt{unicamp-dl/mt5-base-en-pt-msmarco-v2}, a MonoT5 reranker \cite{monot5} trained on pairs of queries and documents in English and Portuguese from the dataset \cite{mmarco}.

MonoT5 is a sequence to sequence reranker that uses T5 models \cite{t5-google} to generate relevance scores between a pair of query and document. T5 models treat all tasks as \textit{text-to-text}, requiring some adaptations for the query/document similarity task. During training, the format \texttt{\textquotesingle Query: \{query\} Document: \{document\} Relevant:\textquotesingle} is used, with labels \texttt{yes} if the document is relevant to the query, and \texttt{no} otherwise. At inference time, the same format as the training data is used to format pairs of queries and documents to feed the model, and a single-token greedy decode is performed. The score is then obtained by calculating the softmax value considering only the tokens \texttt{no} and \texttt{yes}, and selecting the value corresponding to the \texttt{yes} token. Note that the tokens \texttt{no} and \texttt{yes} are the tokens used in the version provided by \cite{mmarco}, but the publication that introduced the MonoT5 architecture, \cite{monot5}, uses the tokens \texttt{false} and \texttt{true}. Figure \ref{fig:monot5} contains an illustration of the MonoT5 architecture's inference process.

\begin{figure}[htb!]
\centering
\includegraphics[width=0.99\linewidth]{pics/monot5.png} 
\caption{MonoT5}
\label{fig:monot5}
\end{figure}

% A busca com reranker foi capaz de melhorar o desempenho inicial do BM25, alcançado o melhor resultado em MRR e Recall@k (k = [3, 5, 7, 9]). Dessa forma, seria o buscador mais indicado para o nosso RAG.

The search with a reranker was able to enhance the initial performance of BM25, achieving the best results in MRR and Recall@k (k = [3, 5, 7, 9]). Therefore, it would be the recommended retriever for our RAG use case and dataset.
